Stablecoins: Survivorship, Transactions Costs and Exchange Microstructure

Stable coins are not very stable. Cash collateralized coins are more stable, but the overall failure rate is similar to tokens that are not designed to be stable. USD Coin, Tether and Dai have the largest Ethereum market shares, and they have an average velocity nearly three times higher than M1. Centralized and decentralized exchanges are the most active nodes and largest holders on the blockchain. Four of the top ten tokens have Herfindahl indices higher than the U.S. banking system. Median gas fees for Tether rose more than twelve times over the last two years, and nearly twenty times for USD Coin. Transactions of under 50,000 USD can generally be done more cheaply offchain. 24 hour exchange turnover in Tether is nearly 60 billion USD. This is comparable to the daily volume at the NYSE and eight times the daily flow in money market mutual funds. Narrow bid-ask spreads and depth have attracted HFT participation approaching 50%

==> tables/cointegration_relations.tex <==

\begin{table}[!h]
\centering
\begin{threeparttable}
\caption{Cointegration Relations}
\label{tab:coint_vector}
\begin{tabular}{@{\extracolsep{0em}}lrrrr@{}}
\toprule
& \multicolumn{4}{c}{Exchange}\\
\cmidrule{2-5}
  & Bitstamp & Coinbase & itBit & Kraken \\
\midrule
Constant & 86.2793&	85.9186	&84.9048&	88.9752 \\
Exchange Basis & -1.0185&	-1.0184&	-1.0181&	-1.0191 \\
%`     &       &       &       &  \\
Futures Error Correction & -0.0019&	-0.0024&	-0.0027	&-0.0030\\
Exchange Error Correction & 0.0078&	0.0060&	0.0056&	0.0062 \\
\bottomrule
\end{tabular}%
\begin{tablenotes}
\small
\item \textit{Note:} This table reports coefficient estimates for the error correction terms among the four spot exchanges and CME.
\end{tablenotes}
\end{threeparttable}
\end{table}

==> tables/cointegration_tests.tex <==

\begin{table}[!h]
    \centering
	\begin{threeparttable}
    \caption{Cointegration Analysis}
    \label{tab:cointegration_tests}
    \begin{tabular}{@{\extracolsep{1em}}l@{\hskip 2em}lrrr@{}}
        \toprule
        \toprule
        \multicolumn{5}{@{}l}{\textit{Panel A: Futures + Four Spot Exchanges}} \\
        \midrule
        Dimension & Test  & \multicolumn{1}{l}{10pct} & \multicolumn{1}{l}{5pct} & \multicolumn{1}{l}{1pct} \\
        \midrule
        $r \leq 4$   & 2.85 & 7.52  & 9.24  & 12.97 \\
        $r \leq 3$   & $29.15^{**}$ & 17.85 & 19.96 & 24.60 \\
        $r \leq 2$   & $546.19^{**}$ & 32.00 & 34.91 & 41.07 \\
        $r \leq 1$   & $1153.85^{**}$ & 49.65 & 53.12 & 60.16 \\
        $r= 0$     & $2034.21^{**}$ & 71.86 & 76.07 & 84.45 \\
        \midrule
        \multicolumn{5}{@{}l}{\textit{Panel B: Futures + Coinbase + Kraken}} \\
        \midrule
        Dimension & Test  & \multicolumn{1}{l}{10pct} & \multicolumn{1}{l}{5pct} & \multicolumn{1}{l}{1pct} \\
        \midrule
        $r \leq 2$  & 2.87 & 7.52  & 9.24  & 12.97 \\
        $r \leq 1$  & $30.24^{**}$ & 17.85 & 19.96 & 24.60 \\
        $r= 0$   & $605.19^{**}$ & 32.00 & 34.91 & 41.07 \\
        \midrule
        \multicolumn{5}{@{}l}{\textit{Panel C: Coinbase BTC and ETH}} \\
        \midrule
        Dimension & Test  & \multicolumn{1}{l}{10pct} & \multicolumn{1}{l}{5pct} & \multicolumn{1}{l}{1pct} \\
        \midrule
        $r \leq 1$  & 3.02 & 7.52 & 9.24 & 12.97 \\
        $r= 0$   & $33.70^{**}$ & 17.85 & 19.96 & 24.60 \\
        \bottomrule
        \bottomrule
    \end{tabular}%
    \begin{tablenotes}
    \footnotesize
    \item \textit{Note:} Cointegration tests are done using a set of five minute returns using the midpoints from the spliced futures contracts and the spot prices from the four exchanges. We use BIC to select lags. 
    \end{tablenotes}
    \end{threeparttable}
\end{table}

==> tables/liquidity_changes_equity_cycle.tex <==

\begin{table}[H]
    \vspace{-2em}
	\centering
	\caption{Liquidity Changes During Equity Trading Cycle}
	\label{tab:liquidity_equity_cycle}
	\scriptsize
	\begin{threeparttable}
		\begin{tabular}{@{\extracolsep{3.8em}}lccccc@{}}
			\toprule
			\toprule
			\multicolumn{6}{@{}l}{\textit{Panel A: Dollar Trading Volume (\$ mn.)}} \\
			\midrule
			& {Bitstamp} & {CME} & {Coinbase} & {Kraken} & {itBit} \\
			\midrule 
  $Intercept$ & 0.296$^{***}$ & 0.852$^{***}$ & 0.561$^{***}$ & 0.395$^{***}$ & 0.103$^{***}$ \\
  & (0.019) & (0.126) & (0.037) & (0.030) & (0.011) \\
  $London$ & 0.169$^{***}$ & 0.579$^{***}$ & 0.001$^{}$ & 0.039$^{}$ & 0.075$^{***}$ \\
  & (0.025) & (0.164) & (0.046) & (0.037) & (0.014) \\
  $Tokyo$ & -0.019$^{}$ & 0.183$^{}$ & 0.024$^{}$ & -0.101$^{***}$ & 0.033$^{***}$ \\
  & (0.023) & (0.140) & (0.043) & (0.034) & (0.013) \\
  $US$ & 0.137$^{***}$ & 0.849$^{***}$ & 0.383$^{***}$ & 0.158$^{***}$ & 0.076$^{***}$ \\
  & (0.027) & (0.181) & (0.050) & (0.040) & (0.015) \\
  & & & & & \\[-2.4ex] 
  \midrule
 Observations & 2,726 & 1,802 & 2,736 & 2,728 & 2,734 \\
 Adjusted $R^2$ & 0.049 & 0.035 & 0.038 & 0.022 & 0.023 \\
			\midrule
			\multicolumn{6}{@{}l}{\textit{Panel B: Trading Volume (BTC)}} \\
			\midrule
			& {Bitstamp} & {CME} & {Coinbase} & {Kraken} & {itBit} \\
			\midrule 
  $Intercept$ & 80.19$^{***}$ & 233.75$^{***}$ & 152.17$^{***}$ & 107.14$^{***}$ & 27.71$^{***}$ \\
  & (5.12) & (34.01) & (9.76) & (8.13) & (2.85) \\
  $London$ & 46.25$^{***}$ & 161.34$^{***}$ & 0.83$^{}$ & 10.82$^{}$ & 20.67$^{***}$ \\
  & (6.73) & (44.30) & (12.29) & (10.02) & (3.86) \\
  $Tokyo$ & -5.04$^{}$ & 51.83$^{}$ & 6.95$^{}$ & -27.12$^{***}$ & 9.35$^{***}$ \\
  & (6.03) & (38.13) & (11.56) & (8.99) & (3.45) \\
  $US$ & 37.00$^{***}$ & 231.09$^{***}$ & 103.32$^{***}$ & 42.33$^{***}$ & 20.50$^{***}$ \\
  & (7.26) & (48.93) & (13.47) & (10.61) & (4.16) \\
  & & & & & \\[-2.4ex] 
  \midrule
 Observations & 2,726 & 1,802 & 2,736 & 2,728 & 2,734 \\
 Adjusted $R^2$ & 0.05 & 0.04 & 0.04 & 0.02 & 0.02 \\
			\midrule
			\multicolumn{6}{@{}l}{\textit{Panel C: Bid-Ask Spreads (bps)}} \\
			\midrule
			& {Bitstamp} & {CME} & {Coinbase} & {Kraken} & {itBit} \\
			\midrule 
  $Intercept$ & 4.381$^{***}$ & 14.755$^{***}$ & 0.584$^{***}$ & 2.835$^{***}$ & 4.460$^{***}$ \\
  & (0.110) & (0.209) & (0.023) & (0.082) & (0.301) \\
  $London$ & -0.298$^{***}$ & -0.312$^{*}$ & 0.079$^{***}$ & -0.229$^{***}$ & -0.193$^{}$ \\
  & (0.115) & (0.185) & (0.029) & (0.087) & (0.251) \\
  $Tokyo$ & -0.860$^{***}$ & -0.210$^{}$ & -0.095$^{***}$ & -0.161$^{}$ & -0.721$^{**}$ \\
  & (0.130) & (0.371) & (0.026) & (0.098) & (0.310) \\
  $US$ & -0.636$^{***}$ & -0.361$^{**}$ & -0.054$^{*}$ & -0.141$^{}$ & -0.832$^{***}$ \\
  & (0.116) & (0.172) & (0.029) & (0.086) & (0.228) \\
  & & & & & \\[-2.4ex] 
  \midrule
 Observations & 2,726 & 1,788 & 2,736 & 2,728 & 2,734 \\
 Adjusted $R^2$ & 0.021 & 0.000 & 0.013 & 0.003 & 0.007 \\
			\midrule
			\multicolumn{6}{@{}l}{\textit{Panel D: Depth (BTC)}} \\
			\midrule
			& {Bitstamp} & {CME} & {Coinbase} & {Kraken} & {itBit} \\
			\midrule
  $Intercept$ & 2.322$^{***}$ & 36.133$^{***}$ & 14.354$^{***}$ & 4.450$^{***}$ & 1.964$^{***}$ \\
  & (0.104) & (0.814) & (0.337) & (0.156) & (0.035) \\
  $London$ & 0.095$^{}$ & 2.230$^{**}$ & 2.378$^{***}$ & -0.044$^{}$ & 0.049$^{}$ \\
  & (0.116) & (0.891) & (0.386) & (0.160) & (0.044) \\
  $Tokyo$ & 0.097$^{}$ & 3.391$^{***}$ & 0.221$^{}$ & 0.369$^{}$ & -0.174$^{***}$ \\
  & (0.131) & (1.074) & (0.444) & (0.280) & (0.044) \\
  $US$ & 0.140$^{}$ & 7.993$^{***}$ & 1.291$^{***}$ & 0.193$^{}$ & 0.123$^{***}$ \\
  & (0.117) & (0.908) & (0.403) & (0.162) & (0.045) \\
  & & & & & \\[-2.4ex] 
  \midrule
 Observations & 2,726 & 1,802 & 2,736 & 2,728 & 2,734 \\
 Adjusted $R^2$ & -0.000 & 0.043 & 0.020 & 0.000 & 0.016 \\
			\bottomrule
			\bottomrule
		\end{tabular}
		\begin{tablenotes}
		\item \textit{Note: } We run five regressions, one for each exchange, on different liquidity measures against trading hours for different regional equity 
		exchanges. The data is aggregated on a half-hourly basis, so each observation corresponds to an exchange, half-hour, and day. 
		The coefficient on the indicator variables is 0 when equity markets at the respective location are open and 1 when they are closed. 
		Tokyo trading hours are from 0:00--6:00 GMT, London trading hours are from 6:00--16:30 GMT, and US  trading hours are from 14:30--21:00 GMT. 
		The sample period is January 1, 2019, to February 28, 2019. CME observations decrease in Panel C. This is because futures going offline cause the CME contract spreads to be undefined; we drop the observations for the half-hours when this occurs.  Robust standard errors are reported in parenthesis. 
		$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01
		\end{tablenotes}
	\end{threeparttable}
\end{table}


==> tables/liquidity_changes_futures.tex <==

\begin{table}[H]
	\centering
	\caption{Liquidity Changes When Futures Go Offline}
	\label{tab:liquidity_futures_offline}
	\small
	\begin{threeparttable}
		\begin{tabular}{@{}lrrrrr@{}}
			\toprule
			\toprule
			\multicolumn{6}{@{}l}{\textit{Panel A: Half-Hourly Dollar Volume (\$ mn.)}} \\
			\midrule
            \midrule
             Exchange &  Online &  Weekday Off &  \textit{t}-stat &  Weekend Off &  \textit{t}-stat \\
            \midrule
Bitstamp &  0.4497 &   0.2904 &     -6.1688 &   0.2709 &     -8.8261 \\
Coinbase &  0.7463 &   0.6546 &     -2.4268 &   0.5200 &     -6.3993 \\
Kraken   &  0.4549 &   0.3978 &     -1.5262 &   0.3666 &     -2.6188 \\
itBit    &  0.1740 &   0.0706 &     -8.7754 &   0.1403 &     -2.7375 \\
			\midrule
			\multicolumn{6}{@{}l}{\textit{Panel B: Half-Hourly Volume (BTC)}} \\
			\midrule
             Exchange &  Online &  Weekday Off &  \textit{t}-stat &  Weekend Off &  \textit{t}-stat \\
            \midrule
Bitstamp &  122.34 &    78.96 &     -6.3117 &    72.95 &     -9.2457 \\
Coinbase &  203.20 &   178.72 &     -2.4002 &   140.03 &     -6.7695 \\
Kraken   &  123.84 &   108.14 &     -1.5669 &    98.54 &     -2.8455 \\
itBit    &   47.44 &    19.04 &     -9.0627 &    37.73 &     -2.9645 \\
			\midrule
			\multicolumn{6}{@{}l}{\textit{Panel C: Average Half-Hourly Bid-Ask Spread (\%)}} \\
			\midrule
            Exchange &  Online &  Weekday Off &  \textit{t}-stat &  Weekend Off &  \textit{t}-stat \\
            \midrule			
Bitstamp &  0.0362 &   0.0602 &      5.8512 &   0.0421 &      5.3961 \\
Coinbase &  0.0055 &   0.0054 &     -0.1969 &   0.0064 &      3.1927 \\
Kraken   &  0.0264 &   0.0343 &      4.1982 &   0.0267 &      0.3854 \\
itBit    &  0.0378 &   0.0840 &      1.7607 &   0.0399 &      2.4227 \\
			\midrule
			\multicolumn{6}{@{}l}{\textit{Panel D: Average Half-Hourly Depth (BTC)}} \\
			\midrule
            Exchange &  Online &  Weekday Off &  \textit{t}-stat &  Weekend Off &  \textit{t}-stat \\
			\midrule
Bitstamp &   2.4996 &   2.2447 &     -1.6468 &   2.2587 &     -2.5329 \\
Coinbase &  16.9006 &   9.8604 &     -9.2269 &  13.2415 &    -11.0271 \\
Kraken   &   4.8591 &   3.8937 &     -2.6512 &   4.0065 &     -5.2418 \\
itBit    &   2.0389 &   2.1911 &      1.3336 &   1.7885 &     -6.2438 \\
			\bottomrule
			\bottomrule
		\end{tabular}
		\begin{tablenotes}
		\item \textit{Note: } We calculate the average half-hourly liquidity for each exchange in three subsamples: when futures are online (\textit{Online}), when futures are offline Monday-Thursday from 22:00-23:00 GMT (\textit{Weekday Off}), and then again from Friday at 22:00  to Sunday at 23:00 (\textit{Weekend Off}). We provide the \textit{t}-statistic  (unequal sample sizes, unequal variances) between the means for the online and two offline  periods. 
		\end{tablenotes}
	\end{threeparttable}
\end{table}


==> tables/liquidity_compare_eth.tex <==
\begin{table}[H]
	\centering
	\begin{threeparttable}
		\caption{Weekday Liquidity Comparison BTCUSD v. ETHUSD}
		\label{tab:eth_liquidity_compare}
		\begin{tabular}{@{\extracolsep{7em}}lrr@{}}
			\toprule
			\toprule
			\multicolumn{3}{@{}l}{\textit{Panel A: Avg. Daily Dollar Volume (\$mn.)}} \\
			\midrule
			Exchange &     BTCUSD &      ETHUSD  \\
			\midrule
Bitstamp &   21.10 &    5.22 \\
Coinbase &   35.43 &   16.89 \\
			\midrule
			\multicolumn{3}{@{}l}{\textit{Panel B: Avg. Daily Volume (BTC,ETH)}} \\
			\midrule
			Exchange &     BTCUSD &      ETHUSD   \\
			\midrule
Bitstamp &  5741.14 &   41076.30 \\
Coinbase &  9650.33 &  130815.08 \\
			\midrule
			\multicolumn{3}{@{}l}{\textit{Panel C: Avg. Daily Bid-Ask Spreads (\%)}} \\
			\midrule
			Exchange &     BTCUSD &      ETHUSD   \\
			\midrule
Bitstamp &  0.0414 &  0.0919 \\
Coinbase &  0.0064 &  0.0286 \\
			\midrule
			\multicolumn{3}{@{}l}{\textit{Panel D: Avg. Daily Depth (\$)}} \\
			\midrule
			Exchange &     BTCUSD &      ETHUSD   \\
			\midrule
Bitstamp &   9,825.00 &   4,269.35 \\
Coinbase &  57,989.87 &  11,758.48 \\
			\bottomrule
			\bottomrule
		\end{tabular}%
		\begin{tablenotes}
			\item \textit{Note:} The data are averages of daily estimates from January 2 to February 28, 2019. Dollar depth is computed by multiplying the first bid/ask quantity by the bid/ask price and then averaging the two. The weekday is Monday-Friday 00:00 to 24:00 GMT.
		\end{tablenotes}
	\end{threeparttable}
\end{table}

==> tables/literature_summary.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[ht]
    \caption{Summary of Digital Asset Microstructure Literature}
    \label{tab:literature_summary}
    \begin{threeparttable}
        \footnotesize
        \begin{tabular}{@{}lP{0.22\textwidth}P{0.15\textwidth}P{0.35\textwidth}P{0.275\textwidth}@{}}
            \toprule
            \toprule
            References & Sample  & Data Source & Markets & Intersecting Concepts      \\[0.5ex] 
            \midrule
            This paper & Jan. 2019 - Feb. 2019 & Exchange message data and API snapshots & CME, Bitstamp, Coinbase, itBit and Kraken & Pre-and post-trade liquidity, price impact, price discovery, cancellation- execution ratios, HFT \\[0.5ex]
            \midrule
            \citet{Alexander} & Dec 2017 - June 2019 & Kaiko, Thomson Reuters Eikon, coinAPI & CME, CBOE, BRR & Price discovery \\[0.5ex]
            \midrule
            \citet{Augustin} & Jul 2016 - Jun 2017, \newline Jan 2018 - Dec 2018 & Kaiko
            & CME, CBOE, Binance, Bitfinex, Bitstamp, Bittrex, BTC-e, Coinbase, Gemini, GateCoin, HitBTC, itBit, Kraken, OKCoin, Poloniex, Quoine & Post-trade liquidity measures, price efficiency \\[0.5ex]
            \midrule
            \citet{Baur} & Dec. 2017 - Oct. 2018 & Bloomberg, Bitcoincharts.com
            & CME, CBOE, Bitstamp & Price discovery \\[0.5ex]
            \midrule
            \citet{Brauneis} & Dec 2017 - Aug 2018 & Exchange API Snapshots
            & Bitfinex, Bitstamp, Coinbase & Trading volume, bid-ask spreads, depth \\[0.5ex]
            \midrule
            \citet{DyhrbergMicro} & Sep 2017 - May 2018 & Exchange API Snapshots
            & GDAX, Gemini, Kraken & Trading volume, trade sizes, bid-ask spreads, depth \\[0.5ex]
            \midrule
            \citet{Dimpfl} & Nov 2016 - Jan 2017 & Bitcoincharts.com
            & Bitcoin.de, Bitstamp, BTC China, BTC-e, Hitbtc, itBit, Kraken, OKCoin & Trading volume, post-trade spreads \\[0.5ex]
            \midrule
            \citet{Ghysels} & Dec 2013 - Sep 2014 & BTC-e API
            & BTC-e & Trading volume, bid-ask spreads \\[0.5ex]
            \midrule
            \citet{HHO} & Dec 2017 - Jun 2019, \newline Daily & Thomson Reuters Datastream
            & CME, CBOE, BRR, Gemini auction & Price discovery \\[0.5ex]
            \midrule
            \citet{Koutmos} & Oct 2013 - Mar 2018, \newline Daily & Bloomberg 
            & Bitfinex & Bid-ask spreads \\[0.5ex]
            \midrule
            \citet{Makarov} & Jan. 2017 - Feb. 2018 & Kaiko, Bitcoincharts.com
            & 34 exchanges including Bitstamp, Coinbase, and Kraken & Trading volume, price impact \\[0.5ex]
            \bottomrule
            \bottomrule
        \end{tabular}
		\begin{tablenotes}
		    \small
			\item \textit{Note:} All papers use tick-level data except those with ``Daily'' in the Sample column. 
		\end{tablenotes}
    \end{threeparttable}
\end{table}

==> tables/mimpact_changes_futures.tex <==


\begin{table}[!h]
	\centering
	\begin{threeparttable}
		\caption{Mann Whitney Tests on Market Impacts}
		\label{tab:market_impact_utest}
		\begin{tabular}{@{\extracolsep{0.5em}}lrrrrr@{}}
			\\[-4ex]
			\toprule 
            Exchange & Weekday & Weekday Off &        U-test p-value & Weekend Off &      U-test p-value \\
            \midrule
            Bitstamp &   0.299 &    0.248 &  0.003 &    0.324 &  0.000 \\
            Coinbase &   0.098 &    0.061 &  0.001 &    0.078 &  0.001 \\
            Kraken   &   0.076 &    0.087 &  0.132 &    0.074 &  0.152 \\
            itBit    &   0.412 &    0.552 &  0.051 &    0.409 &  0.340 \\
			\bottomrule 
		\end{tabular}%
		\begin{tablenotes}
		    \small
			\item \textit{Note:} For each exchange, day, and hour, we estimate Hasbrouck VARs and market impact IRFs. This table summarizes 50-tick market impacts computed from the VARs. We compute medians for three subsamples are: when futures are online (\textit{Online}), when futures are offline Monday-Thursday from 22:00-23:00 GMT (\textit{Weekday Off}), and then again from Friday at 22:00  to Sunday at 23:00 (\textit{Weekend Off}). U-tests are computed between the \textit{Online} subsample and the two offline subsamples. The sample period is January 2, 2019, to March 1, 2019.
		\end{tablenotes}
	\end{threeparttable}
\end{table}


==> tables/pricediscovery_pairwise.tex <==


\begin{table}[!h]
\centering
\begin{threeparttable}
\caption{Pairwise Price Discovery Estimates with Futures}
\label{tab:information_shares}
\begin{tabular}{@{\extracolsep{1em}}lrrrrr@{}}
\toprule
&       &     &   \multicolumn{3}{c}{Information Share}        \\
\cmidrule{4-6}
& \multicolumn{1}{l}{Component Share} &          & \multicolumn{1}{r}{Lower} & \multicolumn{1}{l}{Midpoint} & \multicolumn{1}{l}{Upper} \\
\midrule
Bitstamp & 19.74\%	&  & 0.62\%	& 44.76\%	& 88.89\% \\
Coinbase & 28.66\%	&  & 1.04\%	& 46.59\%	& 92.14\% \\
itBit    & 32.05\%	&  & 1.25\%	& 47.44\%	& 93.63\% \\
Kraken   & 8.91\%	&  & 1.57\%	& 46.67\%	& 91.76\% \\
\bottomrule
\end{tabular}%
\begin{tablenotes}
\small
\item \textit{Note:} The table reports pairwise estimates of price discovery measures using the error correction coefficients for the component shares and the Hasbrouck variance decomposition for the information shares.
\end{tablenotes}
\end{threeparttable}
\end{table}

==> tables/summary_stats_cancels.tex <==

\begin{table}[H]
	\centering
	\caption{Summary Statistics for Cancellation/Execution Ratios for BTCUSD}
	\label{tab:cancellation_execution}
	\small
	\begin{threeparttable}
		\begin{tabular}{@{\extracolsep{1em}}lrrrrrrr@{}}
			\toprule
			\toprule
			\multicolumn{8}{@{}l}{\textit{Panel A: Cancellation/Execution Ratio for All Quotes and Trades}} \\
			\midrule 
			Exchange &     Mean &      StDev  &     Min &     25\% &      50\% &      75\% &       Max \\
			\midrule
            Bitstamp &  50.27 &  17.95 &  24.51 &  35.41 &  48.70 &  55.77 &  113.54 \\
            Coinbase &  36.99 &   7.07 &  21.95 &  33.59 &  36.91 &  39.50 &   67.51 \\
			\midrule
			\multicolumn{8}{@{}l}{\textit{Panel B: HFT Fraction of Cancels (\%)}} \\
			\midrule
			Exchange &     Mean &      StDev  &     Min &     25\% &      50\% &      75\% &       Max \\
			\midrule
			Bitstamp &   8.09 &  2.12 &  3.49 &   6.93 &   7.89 &   9.46 &  15.28 \\
            Coinbase &  15.56 &  5.34 &  5.57 &  11.63 &  15.24 &  18.26 &  35.54 \\
			\bottomrule 
			\bottomrule
		\end{tabular}
		\begin{tablenotes}
		\item \textit{Note: } We assume cancellations within 50 ms of order placement are made by HFT traders. This table summarizes HFT Cancellations as a percentage of all cancellations; the underlying data is aggregated on a daily basis.  Data on order cancels is not available for Kraken or itBit.  The underlying data is aggregated on a daily basis. The sample period is January 1, 2019 to February 28, 2019. 	
		\end{tablenotes}
	\end{threeparttable}
\end{table}

==> tables/summary_stats_mimpacts.tex <==

\begin{table}[!h]
	\centering
	\caption{Summary Statistics for Weekday Hasbrouck Market Impacts (USD) }
	\label{tab:market_impact_statistics}
	\begin{threeparttable}
		\begin{tabular}{@{\extracolsep{1em}}llrrrrrr@{}}
			\\[-4ex]
			\toprule 
            Exchange &  Mean &    StDev &    Min &    25\% &    50\% &    75\% &    Max \\
			\midrule
            Bitstamp &  0.316 &  0.130 &  0.034 &  0.224 &  0.299 &  0.389 &  1.287 \\
            Coinbase &  0.130 &  0.114 &  0.003 &  0.051 &  0.097 &  0.170 &  0.822 \\
            Kraken   &  0.093 &  0.076 &  0.000 &  0.040 &  0.077 &  0.121 &  0.493 \\
            itBit    &  0.508 &  0.414 &  0.001 &  0.216 &  0.412 &  0.689 &  3.807 \\
            CME      &  0.437 &  0.250 &  0.008 &  0.370 &  0.425 &  0.474 &  5.954 \\
			\bottomrule 
    	\end{tabular}%
		\begin{tablenotes}
		\small
		\item \textit{Note:} For each exchange, hour, and day, we fit Hasbrouck VARs with BIC lag selection. This table summarizes cumulative market impact IRFs at the 50th tick computed from the VARs. Market impacts are converted to dollars using the midpoint price for each exchange--hour--day subsample. The sample period consists of weekdays between January 2, 2019, to February 28, 2019, for hours when futures are online. Market impacts outside $(0,10)$ were trimmed. 
		\end{tablenotes}
	\end{threeparttable}
\end{table}

==> tables/summary_stats_weekday_liquidity.tex <==

\begin{table}[H]
	\centering
	\caption{Summary Statistics for Weekday BTCUSD Liquidity}
	\label{tab:liquidity_summary_stats}
	\footnotesize
	\begin{threeparttable}
		\begin{tabular}{@{\extracolsep{1em}}lrrrrrrr@{}}
            \toprule
            \toprule
            \multicolumn{8}{@{}l}{\textit{Panel A: Average Daily Dollar Volume (\$ mn.)}} \\
            \midrule
            Exchange &     Mean &      StDev  &     Min &     25\% &      50\% &      75\% &       Max \\
            \midrule
            Bitstamp &  21.10 &   8.37 &   8.11 &  15.66 &  19.15 &  25.69 &   45.10 \\
            Coinbase &  35.43 &  12.59 &  20.55 &  28.70 &  32.01 &  38.92 &   80.79 \\
            Kraken   &  21.64 &   8.84 &   9.35 &  16.11 &  20.75 &  23.41 &   52.05 \\
            itBit    &   8.08 &   3.65 &   2.00 &   5.86 &   7.42 &   8.95 &   17.44 \\
            All Spot &  86.26 &  31.93 &  41.24 &  67.37 &  80.24 &  94.38 &  193.39 \\
            CME      &  60.10 &  31.34 &   0.96 &  40.75 &  63.07 &  71.76 &  168.71 \\
            \midrule
            \multicolumn{8}{@{}l}{\textit{Panel B: Average Daily Volume (BTC)}} \\
            \midrule
            Exchange &     Mean &      StDev  &     Min &     25\% &      50\% &      75\% &       Max \\
            \midrule
            Bitstamp &   5741 &  2168 &   2376 &   4394 &   5154 &   6865 &  12007 \\
            Coinbase &   9650 &  3254 &   5957 &   7623 &   8775 &  10486 &  21524 \\
            Kraken   &   5894 &  2327 &   2734 &   4499 &   5465 &   6452 &  13894 \\
            itBit    &   2204 &   981 &    586 &   1649 &   1981 &   2340 &   4639 \\
            All Spot &  23489 &  8304 &  12080 &  19123 &  21906 &  24411 &  51544 \\
            CME      &  16531 &  8627 &    275 &  11895 &  17660 &  20025 &  48205 \\
            \midrule
            \multicolumn{8}{@{}l}{\textit{Panel C: Average Trade Size (\$)}} \\
            \midrule
            Exchange &     Mean &      StDev  &     Min &     25\% &      50\% &      75\% &       Max \\
            \midrule
            Bitstamp &   2299.98 &   6723.12 &      0.0 &    107.60 &    543.86 &   2539.54 &  877680.00 \\
            Coinbase &    709.25 &   3477.09 &      0.0 &     20.41 &     75.38 &    315.02 &  271117.32 \\
            Kraken   &   2350.23 &   6186.09 &      0.0 &     89.58 &    511.08 &   2061.40 &  390500.00 \\
            itBit    &   2926.02 &   4854.94 &      0.0 &     81.65 &   1305.79 &   3921.02 &  348710.29 \\
            CME      &  26053.88 &  19236.98 &  16500.0 &  17800.00 &  18775.00 &  33550.00 &  849250.00 \\
            \midrule
            \multicolumn{8}{@{}l}{\textit{Panel D: Average Daily Bid-Ask Spreads (\%)}} \\
            \midrule
            Exchange &     Mean &      StDev  &     Min &     25\% &      50\% &      75\% &       Max \\
            \midrule
            Bitstamp &  0.0414 &  0.0142 &  0.0266 &  0.0317 &  0.0372 &  0.0460 &  0.0965 \\
            Coinbase &  0.0064 &  0.0031 &  0.0027 &  0.0041 &  0.0058 &  0.0080 &  0.0204 \\
            Kraken   &  0.0313 &  0.0110 &  0.0171 &  0.0246 &  0.0309 &  0.0359 &  0.0788 \\
            itBit    &  0.0399 &  0.0108 &  0.0226 &  0.0324 &  0.0388 &  0.0486 &  0.0628 \\
            NBBO     &  0.0023 &  0.0012 &  0.0006 &  0.0015 &  0.0019 &  0.0029 &  0.0055 \\
            CME      &  0.1650 &  0.1313 &  0.1261 &  0.1378 &  0.1419 &  0.1493 &  0.9813 \\
            \midrule
            \multicolumn{8}{@{}l}{\textit{Panel E: Average Daily Depth (BTC)}} \\
            \midrule
            Exchange &     Mean &      StDev  &     Min &     25\% &      50\% &      75\% &       Max \\
            \midrule
            Bitstamp &   2.69 &   0.72 &   1.84 &   2.20 &   2.48 &   3.05 &   5.10 \\
            Coinbase &  15.87 &   5.04 &   5.87 &  13.36 &  15.39 &  18.16 &  27.83 \\
            Kraken   &   4.65 &   1.54 &   2.55 &   3.72 &   4.51 &   5.45 &  10.00 \\
            itBit    &   2.19 &   0.33 &   1.56 &   1.91 &   2.24 &   2.38 &   2.81 \\
            NBBO     &  13.08 &   4.40 &   4.83 &  10.27 &  12.40 &  15.14 &  23.51 \\
            CME      &  38.83 &  12.89 &  13.71 &  28.01 &  38.63 &  49.21 &  61.41 \\
            \bottomrule
            \bottomrule
		\end{tabular}%
		\begin{tablenotes}
		\scriptsize
		\item \textit{Note: } The sample period is January 2, 2019, to February 28, 2019.  The weekday is Monday-Friday 00:00 to 24:00 GMT. ``All Spot'' in Panel A refers to all spot market volume.  The NBBO is the best bid and offer across all four spot exchanges. 
		\end{tablenotes}
	\end{threeparttable}
\end{table}

==> tables/weekday_liquidity_corr.tex <==

\begin{table}[H]
    \vspace{-1em}
	\centering
	\caption{Weekday Correlations for Liquidity Variables}
	\label{tab:liquidity_correlations}
	\scriptsize
	\begin{threeparttable}
		\begin{tabular}{@{\extracolsep{2em}}lccccc@{}}
            \toprule
            \toprule
            \multicolumn{6}{@{}l}{\textit{Panel A: Dollar Volume Correlations}} \\
            \midrule
            &  Bitstamp &  Coinbase &  Kraken &  itBit & CME\\
            \midrule
Bitstamp & 1.000 &  &  &  \\ 
         &  &  &  &  \\[0.75ex]
Coinbase & 0.916 & 1.000 &  &  \\ 
         & (14.05) &  &  &  \\[0.75ex]
Kraken & 0.894 & 0.899 & 1.000 &  \\ 
       & (12.30) & (12.65) &  &  \\[0.75ex]
itBit & 0.819 & 0.875 & 0.835 & 1.000 \\ 
      & (8.80) & (11.12) & (9.36) &  \\
CME & 0.543 & 0.535 & 0.369 & 0.557 & 1.000 \\ 
    & (3.98) & (3.90) & (2.45) & (4.13) &  \\
            \midrule
            \multicolumn{6}{@{}l}{\textit{Panel B: BTC Volume Correlations}} \\
            \midrule
            &  Bitstamp &  Coinbase &  Kraken &  itBit & CME \\
            \midrule
Bitstamp & 1.000 &  &  &  \\ 
         &  &  &  &  \\[0.75ex]
Coinbase & 0.917 & 1.000 &  &  \\ 
         & (14.17) &  &  &  \\[0.75ex]
Kraken & 0.896 & 0.901 & 1.000 &  \\ 
       & (12.44) & (12.80) &  &  \\[0.75ex]
itBit & 0.825 & 0.869 & 0.835 & 1.000 \\ 
      & (8.98) & (10.83) & (9.35) &  \\
CME & 0.574 & 0.559 & 0.407 & 0.595 & 1.000 \\ 
    & (4.32) & (4.15) & (2.74) & (4.56) &  \\
            \midrule
            \multicolumn{6}{@{}l}{\textit{Panel C: Bid-Ask Spread Correlations}} \\
            \midrule
            &  Bitstamp &  Coinbase &  Kraken &  itBit & CME \\
            \midrule
Bitstamp & 1.000 &  &  &  \\ 
         &  &  &  &  \\[0.75ex]
Coinbase & 0.831 & 1.000 &  &  \\ 
         & (9.22) &  &  &  \\[0.75ex]
Kraken & 0.711 & 0.859 & 1.000 &  \\ 
       & (6.23) & (10.33) &  &  \\[0.75ex]
itBit & 0.570 & 0.736 & 0.703 & 1.000 \\ 
      & (4.27) & (6.70) & (6.10) &  \\
CME & -0.163 & 0.039 & 0.038 & -0.013 & 1.000 \\ 
    & (1.02) & (0.24) & (0.23) & (0.08) &  \\
            \midrule
            \multicolumn{6}{@{}l}{\textit{Panel D: Depth Correlations}} \\
            \midrule
            &  Bitstamp &  Coinbase &  Kraken &  itBit & CME\\
            \midrule
Bitstamp & 1.000 &  &  &  \\ 
         &  &  &  &  \\[0.75ex]
Coinbase & 0.099 & 1.000 &  &  \\ 
         & (0.61) &  &  &  \\[0.75ex]
Kraken & -0.042 & 0.036 & 1.000 &  \\ 
       & (0.26) & (0.22) &  &  \\[0.75ex]
itBit & 0.288 & -0.154 & -0.238 & 1.000 \\ 
      & (1.86) & (0.96) & (1.51) &  \\
CME & -0.033 & 0.258 & -0.000 & -0.058 & 1.000 \\ 
    & (0.20) & (1.65) & (0.00) & (0.36) &  \\
            \bottomrule
            \bottomrule			
		\end{tabular}%
		\begin{tablenotes}
		\item \textit{Note: } We report correlation matrices for our three primary liquidity variables across our four spot exchanges and CME. Panel A is the first difference of daily dollar volume.  Panel B is the first difference of daily volume (BTC).  Panel C is the first difference of daily average spreads. Spreads are calculated as a percentage of the midpoint and averaged over each day. Panel D is the first difference in depth at the top bid and ask measured in coins. The $t$-statistics for the
		correlation coefficients are reported in parenthesis. The sample period is January 2, 2019, to February 28, 2019; this is a total of 59 days.  The weekday is Monday-Friday 00:00 to 24:00 GMT.
		\end{tablenotes}
	\end{threeparttable}
\end{table}


